Continuous-Depth Neural Models for Dynamic Graph Prediction

We introduce the framework of continuous-depth graph neural networks (GNNs). Neural graph differential equations (Neural GDEs) are formalized as the counterpart to GNNs where the input-output relationship is determined by a continuum of GNN layers, blending discrete topological structures and differential equations. The proposed framework is shown to be compatible with static GNN models and is extended to dynamic and stochastic settings through hybrid dynamical system theory. Here, Neural GDEs improve performance by exploiting the underlying dynamics geometry, further introducing the ability to accommodate irregularly sampled data. Results prove the effectiveness of the proposed models across applications, such as traffic forecasting or prediction in genetic regulatory networks.

==> sections/6_discussion.tex <==
\section{Discussion}
\paragraph{Unknown topology} Several lines of work concerned with learning the graph structure directly from data exist, either by inferring the adjacency matrix within a probabilistic framework \citep{kipf2018neural} or using a soft--attention \citep{choi2017gram,li2018adaptive,wu2019graph}. In particular, the latter represents a commonly employed approach to the estimation of a dynamic adjacency matrix in spatio--temporal settings. Due to the algebraic nature of the relation between the attention operator and the node features, Neural GDEs are compatible with its use inside the GNN layers parametrizing the vector field. Thus, if an optimal adaptive graph representation $\bm{S}(s, \bZ(s))$ is computed through some attentive mechanism, standard Neural GCDEs can be replaced by $\dot\bZ = \sigma\lc\mathbf{S}\bZ\bm{W}\rc.$
%
\paragraph{Embedding stochasticity into GNNs} Recent works \cite{li2020scalable} showed how the Neural ODE paradigm can be extended to stochastic differential equations \cite{oksendal2003stochastic, kunita1997stochastic}. In the same fashion, one could in principle extend Neural GDEs to the stochastic setting, by defining, e.g. \textit{Stratonovich} graph SDEs in the form
\[ \dd \bZ(s) = f_{\cG}(s, \bZ(s), \theta)\dd s + g_{\cG}(s, \bZ(s), \theta)\dd W(s) \] 
being $W(s)$ a multi--dimensional Weiner process. Such a model, which may still be trained via standard adjoint gradients, would allow Neural GDEs to leverage stochasticity as an inductive bias for, e.g., time series modeling.
%
\paragraph{Addition or removal of nodes}
Neural GDE variants operating on sequences of dynamically changing graphs can, without changes to the formulation, directly accommodate addition or removal of nodes as long as its number remains constant during the flows. In fact, the size of parameter matrix $\bm W$ exclusively depends on the node feature dimension, allowing Neural Hybrid GDEs to accomodate a number of nodes changing in time.
